Popularity and Quality in Social News Aggregators: A Study of Reddit and Hacker News

In this paper we seek to understand the relationship between the online popularity of an article and its intrinsic quality. Prior experimental work suggests that the relationship between quality and popularity can be very distorted due to factors like social influence bias and inequality in visibility. We conduct a study of popularity on two different social news aggregators, Reddit and Hacker News. We define quality as the relative number of votes an article would have received if each article was shown, in a bias-free way, to an equal number of users. We propose a simple poisson regression method to estimate this quality metric from time-series voting data. We validate our methods on data from Reddit and Hacker News, as well the experimental data from prior work. This method works well even though the collected data is subject to common social media biases. Using these estimates, we find that popularity on Reddit and Hacker News is a stronger reflection of intrinsic quality than expected.

==> popularity.tex.old.tex <==
%!TEX root = reddit.tex

In this section we describe the results of the anaylsis using the estimated values for quality and view rates. 


\begin{enumerate}
 
 \item Position bias -> right get richer

 \item Large variation in popularity for ``similar'' quality content

 \item Demonstrate rich-get-richer? \gscomment{this requires more analysis... maybe come back to later} 
 \end{enumerate} 

\subsection{Position Bias}
\label{sec:position_bias}
 Figure \ref{fig:position_bias} shows the estimates view rates of for top 100 positions in each subreddit (for visualization purposes, view rates are normalized such that position 1 of each subreddit has a view rate of 1, i.e. $\pview{1} = 1$). All subreddits demonstrate a very strong position bias towards the top 10 to 15 positions but with the notable exception of r/pics, the view rates flatten out from position 30 onwards. This flat view rate among lower positions is generally consistent with other estimates of position bias \cite{krumme2012quantifying, lerman2014leveraging, craswell2008experimental} but the higher positions have a larger share of the market. Although most subreddits have a similar degree of position bias, r/pics has a much stronger position bias than the other subreddits. We revisit this finding later in this section when discussing the relationship between growth rate and popularity in r/pics. 

\begin{figure}
\begin{subfigure}{0.4\textwidth}
\includegraphics[width=\textwidth]{figures/position_bias}
\end{subfigure}
%\begin{subfigure}{0.25\textwidth}
%\includegraphics[width=\textwidth]{figures/viewrates_top25}
%\end{subfigure}
\caption{Estimated view rates for each top 100 positions of each subreddit. View rates have been normalized such that $\pview{1} = 1$.  }
\end{figure}

\subsection{Popularity vs Quality}

We now turn to the central question of this paper: does popularity on Reddit reflect underlying quality? We measure an article's popularity by an article's max score and best position (see section \ref{sec:data} for definitions). To mitigate some potential bias introduced from the estimation method, we will sometimes normalize an article's growth rate based on the estimated growth rates for other article's that were submitted to the same subreddit on the same day. We perform this scaling so that we avoid a common problem that if May 29th had many more visitors than May 30th, then all articles on May 29th would be estimated to have a higher growth rate than May 30th articles. We perform the following scaling: 
\[ \hat{g}^d_i = \frac{ g^d_i - \bar{g}^d }{g^d_{max} - g^d_{min}}\]
 where $d$ is a particular date and $\bar{g}^d, g^d_{max}, g^d_{min}$ are the mean, maximum, and minimum estimated growth rates for that particular subreddit on that date. The percentile of some article measure, such as best position, refers to its position within the distribution of article measures with a particular subreddit. For example, saying the the max score of this article is in the 80$^{th}$ percentile means that it has a higher max score than 80\% of other articles in the subreddit. For an article's best position, this would actually mean that it has its best position was lower than 80\% of best positions because being closer to 1 is better for positions.  
 
\textbf{Ordinal Performance}
\\ We begin by examining the ordinal relationship between growth rate and popularity. Figure \ref{fig:bestPos_rank_all} shows the relationship between the percentile of an article's normalized growth rate and the percentile of its best position for all subreddits. There's a strong positive correlation between the percentile of an article's growth rate and the percentile of their best position (spearman correlation: $.6054$, p=0), indicating that Reddit's voting mechanism is generally efficient. However, consistent with the findings in \cite{gilbert2013widespread} there's a large number of articles have a high estimated growth rate that do not obtain a high best position, and a significant number of relatively low quality articles that gain significant popularity. 

Another way to formalize this question is to compute what percentage of the top $k\%$ of articles (measured by normalized growth rate) appeared in the top $k\%$ of best positions. We summarize these values for each subreddit in table \ref{table:topk_percent}. 

\begin{table*}[h]
\begin{tabular}{|l|l|l|l|}
\hline
subreddit & top 50\% & top 20\% & top 10\% \\ \hline
pics & 69.8 & 69.1 & 68.4 \\ \hline
news & 69.3 & 72.6 & 66.2 \\ \hline
worldnews & 72.0 & 71.9 & 69.1 \\ \hline
videos & 78.2 & 61.5 & 56.7 \\ \hline
todayilearned & 75.2 & 71.3 & 63.0 \\ \hline
AskReddit & 60.8 & 50.1 & 58.7 \\ \hline
\end{tabular}
\label{table:topk_percent}
\end{table*}



\textbf{Cardinal Performance}
\\ We could ask what is the expected quality of articles that appeared on the front page\footnote{Recall that reddit is paginated by 25 positions.} of a given subreddit. More generally, we could examine the distribution of growth rates of all article's whose best position was in some range $[j_{min}, j_{max}]$?  Figure \ref{fig:allSubs_growthRate_by_pos} shows the mean and standard deviation of normalized growth rates when articles (from all subreddits) are bucketed by every 5 positions (up to position 50). Again there's a general positive correlation between growth rate and best position (pearson correlation of .649 for growth rates and .668 for normalized growth rates). 

All subreddits show a similar trend as above, with the exception of r/pics, shown in figure \ref{blah}. The rise in mean quality from position 30 to position 1 is significantly lower than the rise in other subreddits \gscomment{Show this is not because things seemed to have peaked at 30}. Its also the case that r/pics demonstrates a stronger position bias within these positions relative to the other studied subreddits. One hypothesis is that the increased position bias among these positions inhibits the ability of articles to be ranked in accordance with its merits. Indeed, this is one of the primary implications of the ``rich-get-richer'' theory. 

We examine this theory by comparing how well the observed growth in scores are explained by a pure positional effect and how well they are explained by a pure growth rate effect. 

\gscomment{Need to add the theoretical best possible thing to show that its not a fundamental limit} 



\begin{figure*}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/pics_pos_avgGrowthRate}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/til_pos_avgGrowthRate}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/news_pos_avgGrowthRate}
\end{subfigure}
%\begin{subfigure}{0.3\textwidth}
%\includegraphics[width=\textwidth]{figures/videos_pos_avgGrowthRate}
%\end{subfigure}
\caption{Average growth rate of article by best position, grouped by every 5 position. Shaded area represents give standard deviation of growth rates for each position.  }\label{fig:pos_growthRate_plot}
\end{figure*}




\subsection{Pointwise Estimates}

So far, the metrics we have computed were aggregate measures of popularity, so it may be difficult to interpret how these results the distortion of popularity and quality at any particular moment. In this section, we


This measure gives a theoretical limit on how much Reddit could reasonably improve upon its current ranking if it wanted to maximize the growth rates of its top articles\footnote{We make no claim that Reddit necessarily should do this but its a reasonable goal}. 


is an aggregate measure of popularity, such as what is the .... A separate question is how much could Reddit improve its ranking at any given time if it had perfect knowledge of the quality of articles. 

\begin{equation}
\frac{ \sum_t \sum_{j=1}^k (\qup{i, k} - \qdown{i,k})}{\sum_t \sum_{j=1}^k (\qup{i, k} - \qdown{i,k})}
\end{equation}


% \subsection{Rich Get Richer Dynamics}

% One suggestion of Gilbert \cite{gilbert2013widespread} is that articles go overlooked on Reddit because there's too little voting; specifically, that too few users vote on newly submitted content. Figure \ref{fig:position_bias} certainly evidences this claim as a relatively small fraction of people seem to be voting on articles in lower positions. We suggest another theory which is that there's actually \emph{too much voting}, particularly on the top items; users who only vote on the top positions of each subreddit are the actual users who are helping the rich get richer. We briefly examine this hypothesis that voting on the top positions of a subreddit tends to enforce the status quo. 

% Let $G$ be the distribution over the growth rates of articles that appear in the front page (top 25 positions) of r/pics.  Let $G'$ be the distribution of growth rates of articles weighed by the number of time steps in which the article appeared on the front. For example, if there were two articles that appeared on the front page growth rates of .05 and .1, then $G$ would be a discrete distribution with equal chance of observing .05 or .1. If the first article was on the front page for 1 observation and the latter article was on the front page for 9 observations, then $G'$ would place 10\% of its probability mass on .05 and 90\% on .1.

% $G$, the distribution of growth rates that appear on the front page, is mostly determined by voting that occurs on articles when they do not appear on the front page, while $G'$ is mostly influenced by voting that occurs while on article is on the front page. Figure \ref{fig:dynamics} shows a histogram of $G$ and $G'$, denote blah and blah in the plot, for r/pics. This plot shows that the all of the voting on the front page, which is most of the voting on r/pics, does not actually induce a large change from $G$ to $G'$. 

% \begin{figure}
% \includegraphics[width=.4\textwidth ]{figures/pics_front_dist}
% \label{fig:dynamics}
% \caption{blah}
% \end{figure}










==> robustness.tex <==
%!TEX root = reddit.tex


\begin{figure*}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/pics_r2}
\end{subfigure}
%\begin{subfigure}{0.22\textwidth}
%\includegraphics[width=\textwidth]{figures/til_r2}
%\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/news_r2}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/worldnews_r2}
\end{subfigure}
\caption{$r^2$ values for things.  }\label{fig:r2_plots}
\end{figure*}


One potential problem which might bias estimated qualities and view rates is that higher quality articles are more likely to appear in better positions. Thus we might overestimate view rates for high positions while simultaneously underestimating the quality of the articles that appear there, or vice versa. Although we cannot firmly conclude that this doesn't happen, we present some evidence that this bias is not an overwhelming concern. First the natural dynamics of the ranking ensure that we observe each article in many different positions. While low quality articles are rarely seen in high positions, high quality articles are frequently observed in low positions during the early and later parts of their lifetime. 

In particular we're concerned with the effects of observations from the highest positions (top 10 or so positions) because view rates of those positions are significantly higher than all other positions, as shown in section \ref{sec:position_bias}. We test whether these observations bias our estimates by running two separate estimations: one in which which we use all observations and one in which we discard all observations of high posititions (positions 1-15, or 1-25 for r/pics).  \gsedit{Figure blah shows a scatter plot where the $x$ value is the estimated growth rate of an article when all data is used and the $y$ value is the estimated growth rate when only the lower positions are used. Figure bleh shows a similar plot for estimates of the view rates; the $x$ value is the estimated view rate for a position when all data is used and the $y$ value is the estimated view rate when only data from lower positions is used. Most estimates for are quite close, indicating this estimation method is likely not susceptible to this concern.}








==> tables/subStats_summary.tex <==
\begin{table}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Subreddit & \# articles & \begin{tabular}[c]{@{}l@{}}50\% \\ Score\end{tabular} & \begin{tabular}[c]{@{}l@{}}95\% \\ Score\end{tabular} & \begin{tabular}[c]{@{}l@{}}50\% \\ Pos\end{tabular} & \begin{tabular}[c]{@{}l@{}}95\%\\  Pos\end{tabular} \\ \hline
pics & 2452 & 7 & 248 & 137 & 19 \\ \hline
news & 917 & 9 & 535 & 41 & 5 \\ \hline
worldnews & 1103 & 9 & 629 & 48 & 6 \\ \hline
videos & 1065 & 8 & 1706 & 67 & 5 \\ \hline
todayilearned & 1023 & 35 & 2213 & 64 & 3 \\ \hline
AskReddit & 2219 & 9 & 207 & 70 & 13 \\ \hline
\end{tabular}
\caption{Summary statistics for studied subreddits. Statistics based on filtered articles. }
\label{table:subs}
\end{table}
